The depth of Tsirelson's norm

Tsirelson's norm $\|\cdot \|_T$ on $c_{00}$ is defined as the supremum over a certain collection of iteratively defined, monotone increasing norms $\|\cdot \|_k$. For each positive integer $n$, the value $j(n)$ is the least integer $k$ such that for all $x \in \mathbb{R}^n$ (here $\mathbb{R}^n$ is considered as a subspace of $c_{00}$), $\|x\|_T = \|x\|_k$. In 1989 Casazza and Shura asked what is the order of magnitude of $j(n)$. It is known that $j(n) \in \mathcal{O}(\sqrt{n})$. We show that this bound is tight, that is, $j(n) \in \Omega(\sqrt{n})$. Moreover, we compute the tight order of magnitude for some norms being modifications of the original Tsirelson's norm.

==> a-b-c-draft.tex <==
Let $x:\N\rightarrow \N$ be a non-decreasing function. Define
    \[ \calU_{x} := \{F \subset \N : d:= x(\min F) \ \exists_{E_1,\dots,E_{d}} \ E_1 < \dots < E_{d}, E_i \in \calS , F = \bigcup_{i=1}^d E_i \}. \]
It is a regular family. We will provide upper and lower bounds for this family on $j$. First, let us define
    \[j(a,b;c) := \max\{ j(a+i,b-(c-i)) : i \in [0,c] \}.\]

Fix $\calF := \calU_x$. Clearly, $r(a) = (2^{x(a)} - 1) a$. Also, note that sets $E_i$ can be aligned left, that is first few are full, then there is one non-full and the rest are empty.

\begin{lemma}\label{lem:full-sets-unions}
    If $F \in \calF_{a,b}$ with $F = \bigcup_{i=1}^{x(a)} E_i$ and $b-a > r(a)$, then $\min E_i = |E_i|$ for every $i \in [x(a)-1]$ and $|E_{x(a)}| \in \{\min E_{x(a)} - 1, \min E_{x(a)}\}$.
\end{lemma}
\begin{proof}
    By assumption $F \neq [a,b]$. Suppose that the assertion does not hold. First, suppose that $|E_{x(a)}| = 0$. Then we can add any element, and we are fine. Now, suppose that $\min E_{x(a)} \geq |E_{x(a)}| + 2$. If $E_{x(a)}$ is not an interval then we can add any element. If it is an interval but does not contain $b$ then we can add $b$. Therefore, there is $n^*$ the largest $n$ such that $n \in [a,b] \backslash F$ such that for some $i \in [x(a)-1]$ we have $E_i < n^* < E_{i+1}$ and $n^* = \min E_{i+1} - 1$. If $i+1 = x(a)$, then add $n^*$ and ok. Otherwise, we move everything forward adding $n^*$ and also fine. 
\end{proof}

\begin{lemma}
    If $b-a > r(a)$ and $F \in \calF_{a,b}$ with $F = \bigcup_{i=1}^{x(a)} E_i$, then for each $i \in [x(a)]$ we have
        \[2^{i-1}a \leq \min E_i \leq \left\lfloor\frac{b}{2^{x(a)-i+1}}\right\rfloor + 1.\]
    We can also have (I don't know yet which one I will use)
        \[2^{i-1}a \leq \min E_i \leq \left\lfloor\frac{b}{2^{x(a)-i}}\right\rfloor.\]
\end{lemma}
\begin{proof}
    First, we prove the lower bound by induction on $i$. For $i=1$ the inequality is obvious. Let $i \in [x(1)-1]$. Assume that $2^{i-1}a \leq \min E_i$, then by \cref{lem:full-sets-unions} we have $\min E_i = |E_i|$, thus $2^{i-1}a \leq |E_i|$. Therefore, $2^{i-1}a + (2^{i-1}a-1) \leq \max E_i$, and finally, 
    \[ 2^i a \leq \max E_i + 1 \leq \min E_{i+1}.\]

    We prove the upper bound by the "backward" induction on $i$. Note that it is sufficient to prove the inequality without the "floor" as $\min E_i$ is an integer. First, consider the case of $i = x(a)$. By \cref{lem:full-sets-unions}, we have $|E_{x(a)}| \geq \min E_{x(a)} - 1$, and thus $\max E_{x(a)} \geq \min E_{x(a)} + |E_{x(a)} - 1 \geq 2\min E_{x(a)} - 2$. Recall that $\max E_{x(a)} \leq b$, thus, $b \geq 2\min E_{x(a)} - 2$, this yields $\frac{b}{2} + 1 \geq \min E_{x(a)}$. Now, for the induction step, let $i > 1$, and assume that $\min E_i \leq \frac{b}{2^{x(a)-i+1}} + 1$. By \cref{lem:full-sets-unions} we have $\min E_{i-1} = |E_{i-1}|$, thus 
        \[2 \min E_{i-1} - 1 \leq \max E_{i-1} \leq \min E_i - 1.\]
    This gives $\min E_{i-1} \leq \frac{1}{2} \min E_i$, and finally by inductive assumption
        \[ \min E_{i-1} \leq \frac{1}{2}\left( \frac{b}{2^{x(a)-i+1}} + 1 \right) = \frac{b}{2^{x(a)-(i+1)+1}} + \frac{1}{2} < \frac{b}{2^{x(a)-(i+1)+1}} + 1. \]
\end{proof}

\begin{lemma}
    If $b-a > r(a)$, then
    \[j(a,b) \leq 1 + \max\{j(2^{i-1}a, \left\lfloor\frac{b}{2^{x(a)-i}}\right\rfloor + 1; 2^{i-1}a) : i \in [x(a)] \}.\]
\end{lemma}
\begin{proof}
    Let $x \in c_{00}^+$ be such that $j(x) = j(a,b)$ and let $f$ be such that $f(x) = \|x\|$, and either $f \in W_1$ or $E(f) \in \calF_{a,b}$ (such functional exists by \cref{lem:force:star}). Let $E(f) = \bigcup_{i=1}^{x(a)} E_i$. It is sufficient to prove that for every $i \in [x(a)]$ we have $d(f) \leq 1 + j(2^{i-1}a, \left\lfloor\frac{b}{2^{x(a)-i}}\right\rfloor + 1; 2^{i-1}a)$. We have $f = \frac{1}{2} \sum_{j \in E(f)} f_j$ (with $f_1 < f_2 < \dots$, and $\min\supp f_j = j$), and $d(f) = 1 + \max\{d(f_j) : j \in E(f)\}$. We will prove that for every $j \in E(f)$, if $j \in E_i$, then $d(f_j) \leq j(2^{i-1}a, \left\lfloor\frac{b}{2^{x(a)-i}}\right\rfloor + 1; 2^{i-1}a)$
\end{proof}
This should give some logarithmic bound

==> drafts.tex <==

BELOW: Attempt to have the constant of $2$ instead of $\2sqrt{2}$ in the upper bound.

\begin{lemma}\label{lem:reverse-ineq}
    We have
        \[ j(a,b) \leq 1 + \max \{j(a+t, b-y(a) + t + 1) : t \in [0,y(a)-1]\}.\]
\end{lemma}
\begin{proof}
    Let $j(x) = j(a,b)$ and $f(x) = \|x\|$. If $f \in W_1$, then ok, else $f = \frac{1}{2} \sum_{i=1}^{y(a)} f_i$. We have $d(f) = 1 + \max \{d(f_i) : i \in [y(a)]\}$. Also, $|\supp f_i | \leq |[a,b]| - (y(a)-1)$. Therefore, for each $f_i$ we have
        \[d(f_i) \leq \max\{j(a+t, b-y(a)+t+1) : t \in [0,y(a)-1]\}.\]
\end{proof}

\begin{lemma} \label{lem:recursive}
    If $|[a,b]|\leq y(a)$, then $j(a,b) \leq 1$. Otherwise
        \[j(a,b) \leq 2 + \max\{j(a+i,b-2y(a)+i+2) : i \in [y(a)-1]\} \cup \{1\}.\]
\end{lemma}
\begin{proof}
    The first part follows immediately from \cref{cor:j-small-sets}. We proceed by induction on $b-a$. Suppose that $|[a,b]| > y(a)$. Take a witnessing $x$ (such that $j(a,b) = j(x)$) and $g$ from \cref{lem:upper:main}. We have $j(a,b) = j(x) \leq d(g)$. If $g$ is from \cref{lem:upper:main:i}, then $d(g) = 0$ -- ok. If $g$ is from \cref{lem:upper:main:iv}, then $d(g) \leq j(a+1,b)$. If $|[a+1,b]| \leq y(a+1)$, then $j(a+1,b) \leq 1$ and we are done. Otherwise, by induction we have
        \[j(a+1,b) \leq 2 + \max\{j(a+1+i,b-2y(a+1)+i+2) : i \in [y(a+1)-1]\} \cup \{1\}. \]
    Let $i \in [y(a+1)-1]$. We will show that there exists $i' \in [y(a)-1]$ such that $i'$ contributes to the goal maximum, and the contribution is larger than the one by $i$. If $i \leq y(a)-1$, then we have $[a+1+i,b-2y(a+1)+i+2] \subset [a+i,b-2y(a)+i+2]$ due to the fact that $y$ is a non-decreasing function. By \cref{lem:j-ab:props} this yields $j(a+1+i,b-2y(a+1)+i+2) \leq j(a+i,b-2y(a)+i+2)$ (we ca take $i' := i$). Now suppose that $i > y(a)-1$. Take $i' := y(a)-1$. We have $[a+1+i,b-2y(a+1)+i+2] \subset [a+y(a)-1, b-y(a)+1]$, and we can again apply \cref{lem:j-ab:props}.
    
    Finally, suppose that $g$ is from \cref{lem:upper:main:ii} or \cref{lem:upper:main:iii}. Recall that $E(g) \in \calF_{a,b}$ -- adding the assumption that $|[a,b]| > y(a)$ we obtain $|E(g)| = y(a)$. The same for $E(g_1)$ (if from \cref{lem:upper:main:iii}). First, say that $d(g) = 1 + d(g_{i-1}) \leq 1 + j(\min \supp g_{i-1}, \max \supp g_{i-1})$ for some $i - 1 > 1$. We have $\min \supp g_{i-1} \geq a + i$, and $b-y(a)+i+1 \leq \max \supp g_{i-1}$. To prove the claim, it suffices to find $i' \in [y(a)-1]$ such that
        \[j(a+i, b-y(a)+i+1) \leq 1 + j(a+i', b-2y(a)+i'+2).\]
    Apply \cref{lem:reverse-ineq} to $a' := a+i$ and $b' := b-y(a)+i+1$, we obtain $t \in [y(a')-1]$ such that
        \[ j(a',b') \leq 1 + j(a'+t, b'-y(a')+t+1) = 1 + j(a+i+t, b-y(a)+i+1-y(a+i) + t + 1). \]
    Note that by \cref{lem:j-ab:props} the last expression is bounded by $1 + j(a+i+t, b-2y(a)+i + t+2)$. If $i+t \in [y(a) -1]$, then we can take $i' := i+t$ and we are done. Otherwise, take $i' := y(a)-1$. We have 
        \[ j(a',b') \leq 1 + j(a+i+t, b-2y(a)+i + t+2)  \]
    TODO: problem if $i+t$ large. Fix by hand or prove $t$-monotonicity of $j$.
    It follows that for $h$ being any of $g_i$ or $t_i$ we have  
        \[|\supp h| \leq |[a,b]| - (d-1) = |[a,b]| - y(a) + 1 = b-a-y(a)+2. \]
    Moreover, we know that either $g_1 \in W_1$ or $t_1 \in W_1$. If $d(g) = d(t_1)$ or $d(g) = d(g_1)$, then $d(g) \leq 3$. Otherwise, we obtain the required inequality. (TODO: elaborate, but in a nice way.)
\end{proof}

==> old.computations-for-families.tex <==
\subsection{Modified Schreier}
    Let $y: \N \rightarrow \N$ be non-decreasing satisfying $y(y(u)+v) \geq y(u) + y(v)$, define
        \[\calS_y = \{ F \subset \N : y(\min F) \geq |F|\}\]
    \begin{lemma}\label{lem:S_y:properties}
    We have
        \begin{enumerate}
            \item $\calS_y$ is a regular family, \label{lem:S_y:properties:reg}
            \item $r(n) = y(n)$, \label{lem:S_y:properties:r}
            \item $\calS_y$ is well-aligned, \label{lem:S_y:properties:align}
            \item $\calS_y$ is nice,\label{lem:S_y:properties:nice}
            \item $m(a,b) = y(a) - 2$,\label{lem:S_y:properties:m}
            \item the starting point of $\calS_y$ is $\min y^{-1}([3,\infty))$,\label{lem:S_y:properties:start}
            \item $\calS_y$ is structured.\label{lem:S_y:properties:structured}
        \end{enumerate}
    \end{lemma}
    \begin{proof}
        \cref{lem:S_y:properties:reg} follows from the fact that $y$ is non-decreasing. The only nontrivial property of the remaining is niceness. Let $F = \{n_1,n_2,\dots,n_{|F|}\}, G = \{m_1,m_2,\dots,m_{|G|}\} \in \calS_y$ such that 
    \begin{itemize}
        \item $n_1 = m_1$,
        \item $m_{|G|} < n_2$,
        \item $m_2 - m_1 + 1 > r(n_1)$.
    \end{itemize}
    We need to prove that
        \[H := \{m_2,m_3,\dots,m_{|G|},n_2,\dots,n_{|F|} \} \in \calS_y.\]
    In other words, we need $y(m_2) \geq |F| + |G| - 2$. We apply the function $y$ to the third assumption getting
        \[ y(m_2) \geq y(y(n_1) + m_1) \geq y(n_1) + y(m_1) \geq |F| + |G| > |F| + |G| - 2. \qedhere \]
    \end{proof}

\subsection{Unions of Schreier}
    Let $k \in \N, k\geq 2$, and define
        \[k\calS_1 = \{F \subset \N : \exists_{E_1,\dots,E_k \in \calS_1} \ F = \bigcup_{i=1}^k E_i\}.\]
    \begin{lemma}\label{lem:kS_1:properties}
    We have
        \begin{enumerate}
            \item $k\calS_1$ is a regular family, \label{lem:kS_1:properties:reg}
            \item $r(n) = (2^k-1)n$, \label{lem:kS_1:properties:r}
            \item $k\calS_1$ is well-aligned, \label{lem:kS_1:properties:align}
            \item $k\calS_1$ is nice,\label{lem:kS_1:properties:nice} [ACTUALLY, I DON'T THINK SO... :(]
            \item $m(a,b) \geq b+a- \lfloor\frac{b+1}{2^{k-1}}\rfloor - 1$,\label{lem:kS_1:properties:m}
            \item the starting point of $k \calS_1$ is $1$,\label{lem:kS_1:properties:start}
            \item $k \calS_1$ is structured.\label{lem:kS_1:properties:structured}
        \end{enumerate}
    \end{lemma}
    \begin{proof}
        
    \end{proof}

==> old.families-results.tex <==
Current status:
\begin{itemize}
    \item $\calA_k \Rightarrow j(n) = \Theta(\frac{n}{k})$,
    \item $\calS \Rightarrow j(n) = \Theta(\sqrt{n})$, $[\sqrt{2n}-3 \leq j(n) \leq \sqrt{8n}+3]$ (better bound using the other paper -- $j(n) \leq \sqrt{4n} + c $
    \item $\calS_y \Rightarrow j(n) = \Theta((\sum_{i=1}^ny(i))^{-1})$,
    \item $k\calS \Rightarrow j(n) = \Theta(\frac{1}{k} \log n)$,
    \item $\calS k = S_{x \mapsto kx} \Rightarrow j(n) = \Theta(\frac{1}{k} \sqrt{n})$,
    \item $\calS_2 \Rightarrow j(n) = \Theta(\sqrt{\log n})$ $[\sqrt{2\log n}  - 4 \leq j(n) \leq  8 \sqrt{\log n} + 34]$
\end{itemize}
